Decentralized Singular Value Decomposition for Large-scale Distributed Sensor Networks

This article studies the problem of decentralized Singular Value Decomposition (d-SVD), which is fundamental in various signal processing applications. Two scenarios are considered depending on the availability of the data matrix under consideration. In the first scenario, the matrix of interest is row-wisely available in each local node in the network. In the second scenario, the matrix of interest implicitly forms an outer product from two different series of measurements. By combining the lightweight local rational function approximation approach with parallel averaging consensus algorithms, two d-SVD algorithms are proposed to cope with the two aforementioned scenarios. We evaluate the proposed algorithms using two application examples: decentralized sensor localization via low-rank matrix completion and decentralized passive radar detection. Moreover, a novel and non-trivial truncation technique, which employs a representative vector that is orthonormal to the principal signal subspace, is proposed to further reduce the communication cost associated with the d-SVD algorithms. Simulation results show that the proposed d-SVD algorithms converge to the centralized solution with reduced communication cost compared to those facilitated with the state-of-the-art decentralized power method.

==> dRecmendation.tex <==
\subsection{Distributed recommendation system design}\label{subsec:rec}
Recommendation systems are effective filtering tools in the big data era to provide content of interest, e.g., books, movies, and music, for users. Approaches to design recommendation systems are categorized into the content-based approach, the collaborative filtering approach, and the hybrid approach \cite{mehtaReviewmatrix2017}. On the one hand, in the content-based approach, the recommendation is made based on the user's own information, e.g., tags, video or audio stream, in the past \cite{mehtaReviewmatrix2017}. On the other hand, the collaborative filtering approach collects ratings of items from different users into the user-item rating matrix and make the recommendation collaboratively \cite{chenSurveycollaborative2018}. As the user-item rating matrices are generally sparse and low-rank, low-rank matrix completion techniques, such as the SVD-based Singular Value Thresholding (SVT) algorithm, can be applied to design recommendation systems to predict unknown user-item ratings \cite{zhangMatrixCompletion2022}.
% Among the collaborative filtering approaches, the SVD-based matrix factorization methods are model-based methods that collects ratings of items from different users into the sparse user-item rating matrix and factorizes it into user feature and item feature matrices to predict unknown user-item ratings \cite{chenSurveycollaborative2018}. 

As the number of users and items increases drastically in last decades, three difficulties arise in designing recommendation systems. First, large storage cost to maintain the user-item rating matrix at the fusion center. Second, high bandwidth requirement to collect all user-item ratings to the fusion center. Third, the privacy concern on sharing private ratings with the fusion center. Hence, a distributed recommendation system that does not need to collect the rating data at a fusion center is preferable. In such a case, the large storage cost and high bandwidth requirement at the fusion center are avoided, and the privacy of each user can be improved\footnote{Extra operation is needed to guarantee the privacy, such as using the privacy preserved average consensus algorithm \cite{liPrivacypreservingdistributed2020,liPrivacypreservingdistributed2022}.}. 

In this section, we design a fully distributed recommendation system based on the SVT algorithm by utilizing our d-SVD algorithm proposed in Section \ref{sec:dSVDknonw}. Specifically, based on the sparse rating matrix, denoted as $\widehat{\bR}$, we design the distributed SVT (d-SVT) algorithm to predict unknown ratings. In the rest of this section, we assume that $\widehat{\bR}$ has the dimension $N \times N_2$ with $N\ll N_2$, and is row-wisely partitioned, i.e., each node has one row (or multiple rows) of $\widehat{\bR}$.

\paragraph{Distributed Singular Value Thresholding (d-SVT)} The SVT algorithm consists in the following updates
\begin{subnumcases}{\label{equ:svt}}
	\widetilde{\bR}(t) = \mathcal{D}_\tau\left(\bR(t-1)\right),\label{subequ:shrink}\\
	\bR(t) = \bR(t-1) + \mu\left(\widehat{\bR} - \widetilde{\bR}(t)\odot \bF\right),\label{subequ:update}
\end{subnumcases}
where $t = 1,2,\ldots$, is the iteration index, $\bR(t)$ is an intermediate variable with $\bR(0) = \widehat{\bR}$, $\mu$ is the step size, $\mathcal{D}_\tau(\cdot)$ is the so-called shrinkage operator with the thresholding level $\tau$, and $\bF$ is an indicator matrix that is defined as
\begin{equation}
	f_{ij} = \begin{cases}
		1, & \text{if } \hat{r}_{ij} \text{ is available},\\
		0, & \text{otherwise}.
	\end{cases}
\end{equation}
Denote $\sigma_n(t), n = 1,\ldots,N$, as the singular values of $\bR(t)$ and $\bU(t)\in\mathbb{C}^{N\times N}$ and $\bV(t)\in\mathbb{C}^{N_2\times N}$ as the economy-size left and right singular vector matrix, respectively. The shrinkage operator applied to $\bR(t)$ is defined as \cite{caiSingularvalue2010}
\begin{equation}\label{equ:shrinkage}
	\mathcal{D}_{\tau}\left(\bR(t)\right) = \sum_{n=1}^{N}[\sigma_n(t) - \tau]^+\bU(t)\bV(t)^\tH,
\end{equation}
where $[\sigma_n(t) - \tau]^+ = \max\left(0,\sigma_n(t)-\tau\right)$. The SVT algorithm terminates when the maximum number of iterations is reached, and returns $\widetilde{\bR}(t)$ as the estimated dense matrix.

Since the update of $\bR(t)$ in \eqref{subequ:update} is performed elementwise, each node maintains one row (or multiple rows) of $\bR(t)$. This satisfies the setup in Section \ref{sec:dSVDknonw}. Hence, the SVD of $\bR(t)$ can be obtained by applying our proposed d-SVD algorithm in a fully decentralized manner. As a result, each node knows complete singular values, one row (or multiple rows) of $\bU(t)$ corresponding to the node index, and complete $\bV(t)$. Thus, the shrinkage operation in \eqref{equ:shrinkage} can be performed locally. Moreover, since the product $\bU(t)\bV(t)^\tH$ instead of the matrix $\bV(t)$ itself is required to perform the shrinkage operation, we can carry out the multiplication of $\bU(t)$ with $\bV(t)^\tH$ once a row of $\bV(t)$ is obtained via \eqref{equ:XUvnk} to reduce the storage cost in each node. As \eqref{subequ:shrink} can be carried out fully distributively and \eqref{subequ:update} involves only local operation, \eqref{equ:svt} is resulted in a distributed SVT algorithm, denoted as d-SVT, by utilizing our proposed d-SVD algorithm in Section \ref{sec:dSVDknonw}.

%From \eqref{equ:svt} and \eqref{equ:shrinkage} we observe that the SVD plays a key role in the SVT algorithm, where our proposed d-SVD algorithm can be applied.

%Observing that the update of $\bR(t)$ in \eqref{subequ:update} is performed elementwise, thus, each sensor knows one row (or one column since $\bR(t)$ is always symmetric) of $\bR(t)$. Hence, the SVD of $\bR(t)$ can be carried out by applying our proposed d-SVD algorithm in Section \ref{sec:dSVDknonw} in a fully decentralized manner. Nevertheless, as $\bR(t)$ is a square matrix, 
%We assume for the distributed recommendation system design that each node maintains all singular values in $\bSigma(t)$, one row (or multiple rows) of $\bU(t)$ and one column (or multiple columns) of $\bV(t)$ that are associated with the node index. Moreover, noticing that only those entries in $\widetilde{\bR}(t)$ associated with neighboring nodes are required to update $\bR(t)$, and examining the matrix multiplication in \eqref{equ:shrinkage}, we observe that the required entries can be easily computed by direct information exchange between neighboring nodes, as direct communication links between them exist. Hence, the SVT algorithm in \eqref{equ:svt} can be realized fully distributively, denoted as d-SVT, by utilizing our proposed d-SVD algorithm in Section \ref{sec:dSVDknonw}.

%\begin{remark}
%	Since $\bR(t)$ is a real matrix, its left and right singular vectors associated with the same singular value are equal up to a real scaling factor, i.e., $\bV(t) = \bU(t)\bDelta(t)$, where $\bDelta(t) = \diag{\delta_1(t),\ldots,\delta_N(t)}$ and $\delta_{n}(t) = \pm 1, \forall n = 1,\ldots,N$.
%\end{remark}

\paragraph{Experimental results} We use the MovieLens-latest-small \cite{harperMovieLensdatasets2016} dataset to validate the d-SVT algorithm. The dataset contains $100836$ ratings across $9742$ movies created from $610$ users. Ratings are scaled from $0.5$ to $5$ with $0.5$ interval and are stored in the matrix $\bar{\bR}\in\mathbb{R}^{610\times 9742}$ with $\bar{r}_{ij}$ denoting the rating from the $i$th user on the $j$th movie. $\bar{r}_{ij} = 0$ if the $i$th user does not have rating on the $j$th movie. We randomly select $40\%$ and $80\%$ of the ratings as the training set and store them in the sparse rating matrix $\widehat{\bR}$. The remaining $60\%$ and $20\%$ of ratings, respectively, are the test sets which can be predicted by applying the proposed d-SVT algorithm.

To have a distributed setup, we split the selected sparse rating matrix $\widehat{\bR}$ row-wisely into $10$ clusters, with each cluster serves as a node that contains ratings created from non-overlapping $61$ users for all movies. The connection of all clusters forms a network that can be represented by Fig.~\ref{fig:networkRecommendation}.
\begin{figure}[t]
	\centering
	\input{simulations/network_recommendation}
	\caption{Distributed clusters for recommendation system. Each cluster contains ratings created from non-overlapping $61$ users for all movies.}
	\label{fig:networkRecommendation}
\end{figure}

% an Erd\H os R\'enyi graph which is generated with $10$ nodes with initial degree $4$ and the connection is rewired with probably $0.1$. (can provide a graph instead the description)

For the d-SVT algorithm, we have $\tau=5N$, the step size $\mu=1.5$, and the maximum iteration of the SVT algorithm is $100$. The iteration of the PS algorithm for the consensus is $50$. The entries of the estimated result $\widetilde{\bR}(t)$ are bounded between $0$ and $5$, and are rounded to the nearest half value, e.g., $0, 0.5, 1, 1.5, \ldots$. The relative error is defined as
\begin{equation}
	\epsilon(t) = \frac{\norm{\widetilde{\bR}(t)\odot\bar{\bF}-\bar{\bR}\odot\bar{\bF}}_\mathtt{fro}}{\norm{\bar{\bR}\odot\bar{\bF}}_\mathtt{fro}},
\end{equation}
where $\bar{\bF}$ is an indicator matrix defined as
\begin{equation}
	\bar{f}_{ij} = \begin{cases}
		1, & \text{if } \bar{r}_{ij} \text{ is from the test set},\\
		0, & \text{otherwise}.
	\end{cases}
\end{equation}

The d-PM and the SGD methods are implemented as comparisons, where the iterations of the PM and the SGD method are set to be $10$ and $500$, respectively.
The simulation result is shown in Fig.~\ref{fig:distrec}.
\begin{figure}[t]
	\centering
	\input{simulations/distrecAll}
	\caption{Relative error performance of d-SVT algorithm for the distributed recommendation system design with different training sizes.}
	\label{fig:distrec}
\end{figure}

\red{TODO}: Comparison with d-PM and potential with \cite{hegedusFullydistributed2014a}. (The total communication cost of d-PM is less than d-EVD for the d-SVT. The reason is that the SVT only requires dominate singular vectors, thus, the d-PM does not need to perform the complete SVD. If complete SVD is considered, the communication cost of the d-PM is much larger as discussed in Section \ref{subsec:dSVDknownCost}. We may add the truncated version of the rational function approaximation, which is under testing.)

truncated $\bA$ and $\bB$: Create $\bA=\bU_s\bar{\bA}$ for fixed $\bU_s$ and random $\bar{\bA}\in\mathbb{C}^{M\times N}$. $\bB$ can be full rank or alternatively, also low-rank. 
